Defending Against Physically Realizable Attacks on Image Classification

We study the problem of defending deep neural network approaches for image classification from physically realizable attacks. First, we demonstrate that the two most scalable and effective methods for learning robust models, adversarial training with PGD attacks and randomized smoothing, exhibit very limited effectiveness against three of the highest profile physical attacks. Next, we propose a new abstract adversarial model, rectangular occlusion attacks, in which an adversary places a small adversarially crafted rectangle in an image, and develop two approaches for efficiently computing the resulting adversarial examples. Finally, we demonstrate that adversarial training using our new attack yields image classification models that exhibit high robustness against the physically realizable attacks we study, offering the first effective generic defense against such attacks.

==> adversarial_patch.tex <==
\section{Adversarial Patch}

Other than specific attacks on these two tasks, we also choose a universal adversarial patch attack on Face Recognition task and traffic sign task. 



\subsection{Face Recognition }
We used 27 images (9 classes * 3 images in each class)  to design the universal adversarial patch. 



% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}[H]
\centering 
\caption{Best Result Comparison between Different Methods against Adversarial Patch}
\label{tab:Main}
\begin{tabular}{@{}ccccccc@{}}
\toprule
                                                                & \multicolumn{6}{c}{Attacking Region}                                                                      \\ \cmidrule(l){2-7} 
                                                                & 0\%             & 5\%             & 10\%            & 15\%            & 20\%            & 25\%            \\ \midrule
\multicolumn{1}{c|}{Clean Model}                                & 98.34\%         & 80.69\%         & 41.21\%         & 19.41\%         & 9.76\%          & 5.75\%          \\
\multicolumn{1}{c|}{Adv. Training: $\eps$ = 8/255}             & 65.53\%         & 21.58\%         & 19.85\%         & 18.11\%         & 17.14\%         & 16.05\%         \\
\multicolumn{1}{c|}{Randomized Smoothing: $\sigma$ = 1}         & 92.98\%         & 61.99\%         & 36.26\%         & 33.80\%         & 24.68\%         & 16.02\%         \\
\multicolumn{1}{c|}{($100\times50$)Exhaustive Search with 50 PGD} & \textbf{98.7\%} & \textbf{98.7\%} & \textbf{97.8\%} & \textbf{97.2\%} & \textbf{81.2\%} & 24.2\%          \\
\multicolumn{1}{c|}{($70\times70$)Exhaustive Search with 50 PGD}  & 98.5\%          & 98.4\%          & 97.3\%          & 96.5\%          & 63.2\%          & \textbf{44.1\%} \\ \bottomrule
\end{tabular}
\end{table}


\begin{table}[H]
\centering
\caption{Adversarial Training against Adversarial Patch}
\label{tab:Adv_patch}
\begin{tabular}{@{}ccccccc@{}}
\toprule
                                                                 & \multicolumn{6}{c}{Attacking Region}                                                                            \\ \cmidrule(l){2-7} 
                                                                 & 0\%              & 5\%              & 10\%             & 15\%             & 20\%             & 25\%             \\ \midrule
\multicolumn{1}{c|}{Clean Model}                                 & \textbf{98.34\%} & \textbf{80.69\%} & 41.21\%          & 19.41\%          & 9.76\%           & 5.75\%           \\ \midrule
\multicolumn{1}{c|}{7 Iterations Adv. Training: $\eps$ = 4/255}  & 89.36\%          & 57.05\%          & 39.15\%          & 34.71\%          & 10.52\%          & 7.81\%           \\
\multicolumn{1}{c|}{7 Iterations Adv. Training: $\eps$ = 8/255}  & 67.02\%          & 27.98\%          & 23.54\%          & 21.26\%          & 18.55\%          & \textbf{17.03\%} \\ \midrule
\multicolumn{1}{c|}{50 Iterations Adv. Training: $\eps$ = 4/255} & 89.36\%          & 57.38\%          & \textbf{53.58\%} & \textbf{36.01\%} & \textbf{28.85\%} & 16.05\%          \\
\multicolumn{1}{c|}{50 Iterations Adv. Training: $\eps$ = 8/255} & 65.53\%          & 21.80\%          & 21.15\%          & 17.79\%          & 17.79\%          & 16.70\%          \\ \bottomrule
\end{tabular}
\end{table}



\begin{table}[H]
\centering 
\caption{Curriculum Adversarial Training against Adversarial Patch}
\label{tab:CAdv_patch}
\begin{tabular}{ccccccc}
\hline
                                                     & \multicolumn{6}{c}{Attacking Region}                                                                            \\ \cline{2-7} 
                                                     & 0\%              & 5\%              & 10\%             & 15\%             & 20\%             & 25\%             \\ \hline
\multicolumn{1}{c|}{Clean Model}                     & \textbf{98.34\%} & 80.69\%          & 41.21\%          & 19.41\%          & 9.76\%           & 5.75\%           \\
\multicolumn{1}{c|}{CAdv. Training: $\eps$ = 4/255}  & 97.02\%          & \textbf{52.49\%} & \textbf{45.44\%} & 30.91\%          & 16.05\%          & 10.85\%          \\
\multicolumn{1}{c|}{CAdv. Training: $\eps$ = 8/255}  & 96.17\%          & 44.79\%          & 29.18\%          & 23.86\%          & 12.47\%          & 10.20\%          \\
\multicolumn{1}{c|}{CAdv. Training: $\eps$ = 16/255}  & 90.63\%          & 48.26\%          & 34.38\%          & 28.85\%          & 23.54\%          & \textbf{19.20\%} \\
\multicolumn{1}{c|}{CAdv. Training: $\eps$ = 32/255} & 80.85\%          & 42.95\%          & 40.46\%          & \textbf{32.00\%} & \textbf{20.93\%} & 17.14\%          \\ \hline
\end{tabular}
\end{table}





\begin{table}[H]
\centering
\caption{Randomized Smoothing against Adversarial Patch}
\label{tab:RS_patch}
\begin{tabular}{@{}ccccccc@{}}
\toprule
                                                           & \multicolumn{6}{c}{Attacking Region}                                                                           \\ \cmidrule(l){2-7} 
                                                           & 0\%              & 5\%              & 10\%             & 15\%             & 20\%             & 25\%            \\ \midrule
\multicolumn{1}{c|}{Clean Model}                           & 98.34\%          & 80.69\%          & 41.21\%          & 19.41\%          & 9.76\%           & 5.75\%          \\
\multicolumn{1}{c|}{Randomized Smoothing: $\sigma$ = 0.25} & \textbf{98.72\%} & 60.35\%          & 26.67\%          & 13.80\%          & 6.67\%           & 5.15\%          \\
\multicolumn{1}{c|}{Randomized Smoothing: $\sigma$ = 0.5}  & 97.66\%          & \textbf{81.05\%} & \textbf{58.83\%} & \textbf{33.92\%} & 26.55\%          & 14.74\%         \\
\multicolumn{1}{c|}{Randomized Smoothing: $\sigma$ = 1}    & 92.98\%          & 61.99\%          & 36.26\%          & 33.80\%          & \textbf{24.68\%} & \textbf{16.02\%} \\ \bottomrule
\end{tabular}
\end{table}




\begin{table}[H]
\centering
\caption{Sticker Retraining against Adversarial Patch}
\label{tab:Sticker_patch}
\begin{tabular}{@{}ccccccc@{}}
\toprule
                                                                    & \multicolumn{6}{c}{Attacking Region}                                                                            \\ \cmidrule(l){2-7} 
                                                                    & 0\%              & 5\%              & 10\%             & 15\%             & 20\%             & 25\%             \\ \midrule
\multicolumn{1}{c|}{Clean Model}                                    & 98.34\%          & 80.69\%          & 41.21\%          & 19.41\%          & 9.76\%           & 5.75\%           \\
\multicolumn{1}{c|}{($100\times50$)Exhaustive Search with 50 PGD}     & 98.72\%          & \textbf{98.70\%} & \textbf{97.83\%} & \textbf{97.18\%} & 81.24\%          & 24.19\%          \\
\multicolumn{1}{c|}{($100\times50$)Gradient Based Search with 50 PGD} & 98.51\%          & 98.41\%          & 96.75\%          & 87.42\%          & 57.48\%          & 24.62\%          \\
\multicolumn{1}{c|}{($70\times70$)Exhaustive Search with 50 PGD}      & 98.51\%          & 98.37\%          & 97.29\%          & 96.53\%          & 63.23\%           & \textbf{44.14\%} \\
\multicolumn{1}{c|}{($70\times70$)Gradient Based Search with 50 PGD}  & \textbf{98.94\%} & 97.51\%          & 96.31\%          & 93.82\%          & \textbf{92.19\%} & 31.34\%          \\ \bottomrule
\end{tabular}
\end{table}










\subsection{Traffic Sign }
We used 16 images (16 classes * 1 image in each class)  to design the universal adversarial patch. 


\begin{table}[H]
\centering
\caption{Best Result Comparison between Different Methods against Adversarial Patch}
\label{tab:RS_sign_patch}
\begin{tabular}{@{}ccccccc@{}}
\toprule
                                                                & \multicolumn{6}{c}{Attacking Region}                                                                                       \\ \cmidrule(l){2-7} 
                                                                & 0\%              & 5\%              & 10\%             & 15\%             & 20\%             & 25\%                        \\ \midrule
\multicolumn{1}{c|}{Clean Model}                                & \textbf{98.69\%} & 75.87\%          & 58.62\%          & 40.68\%          & 33.10\%          & 22.47\%                     \\
\multicolumn{1}{c|}{CAdv. Training: $\eps$ = 16/255} & 96.95\%          & 86.93\% & 70.21\%& 66.11\% & 51.13\% &  40.77\%   \\
\multicolumn{1}{c|}{Randomized Smoothing: $\sigma$ = 0.5}       & 96.28\%          & 83.28\% & 68.17\% & 53.86\%          & 48.79\% & \multicolumn{1}{l}{33.10\%} \\
\multicolumn{1}{c|}{(($7\times7$)Gradient Based Search with 30 PGD}  & 95.82\%          & \textbf{90.68\%}         & 88.41\% & \textbf{81.79\%} & \textbf{72.30\%} & \textbf{58.71\%}     \\
\multicolumn{1}{c|}{($7\times7$)Gradient Based Search with 50 PGD}  & 95.82\%          & 90.33\%          & \textbf{89.29\%} & 78.92\% & 70.21\% & 58.54\%           \\ \bottomrule
\end{tabular}
\end{table}




\begin{table}[H]
\caption{Adversarial Training against Adversarial Patch}
\label{tab:RS_sign_patch}
\begin{tabular}{@{}ccccccc@{}}
\toprule
                                                     & \multicolumn{4}{c}{Attacking Region}                                                                                                \\ \cmidrule(l){2-7} 
                                                     & 0\%              & 5\%              & 10\%             & 15\%             & 20\%             & 25\%                                 \\ \midrule
\multicolumn{1}{c|}{Clean Model}                     & 98.69\%          & 75.87\%          & 58.62\%          & 40.68\%          & 33.10\%          & 22.47\%                              \\
\multicolumn{1}{c|}{Adv. Training: $\eps$ = 4/255}   & \textbf{99.04\%} & \textbf{82.14\%} & \textbf{64.46\%} & 45.73\%          & 31.36\%          & 23.78\%                              \\
\multicolumn{1}{c|}{Adv. Training: $\eps$ = 8/255}   & 96.60\%          & 76.74\%          & 62.89\%          & \textbf{46.60\%} & \textbf{37.37\%} & \multicolumn{1}{l}{\textbf{25.09\%}} \\ \bottomrule
\end{tabular}
\end{table}



\begin{table}[H]
\centering
\caption{Curriculum Adversarial Training against Adversarial Patch}
\label{tab:CAdv_sign_patch}
\begin{tabular}{@{}ccccccc@{}}
\toprule
                                                     & \multicolumn{6}{c}{Attacking Region}                                                                                       \\ \cmidrule(l){2-7} 
                                                     & 0\%              & 5\%              & 10\%             & 15\%             & 20\%             & 25\%                        \\ \midrule
\multicolumn{1}{c|}{Clean Model}                     & 98.69\%          & 75.87\%          & 58.62\%          & 40.68\%          & 33.10\%          & 22.47\%                     \\
\multicolumn{1}{c|}{CAdv. Training: $\eps$ = 4/255}  & \textbf{99.13\%} & 77.18\%          & 57.32\%          & 39.02\%          & 38.94\%          & 31.10\%                     \\
\multicolumn{1}{c|}{CAdv. Training: $\eps$ = 8/255}  & 98.72\%          & 86.24\%          & 68.64\%          & 60.19\%          & 42.42\%          & \multicolumn{1}{l}{35.10\%} \\
\multicolumn{1}{c|}{CAdv. Training: $\eps$ = 16/255} & 96.95\%          & \textbf{86.93\%} & \textbf{70.21\%} & \textbf{66.11\%} & \textbf{51.13\%} & \textbf{40.77\%}            \\
\multicolumn{1}{c|}{CAdv. Training: $\eps$ = 32/255} & 97.66\%          & 59.93\%          & 51.57\%          & 45.38\%          & 37.37\%          & 27.79\%                     \\ \bottomrule
\end{tabular}
\end{table}




\begin{table}[H]
\centering 
\caption{Randomized Smoothing against Adversarial Patch}
\label{tab:RS_sign_patch}
\begin{tabular}{@{}ccccccc@{}}
\toprule
                                                           & \multicolumn{5}{c}{Attacking Region}                                                                                       \\ \cmidrule(l){2-7} 
                                                           & 0\%              & 5\%              & 10\%             & 15\%             & 20\%             & 25\%                        \\ \midrule
\multicolumn{1}{c|}{Clean Model}                           & \textbf{98.69\%} & 75.87\%          & 58.62\%          & 40.68\%          & 33.10\%          & 22.47\%                     \\
\multicolumn{1}{c|}{Randomized Smoothing: $\sigma$ = 0.25} & 98.22\%          & 82.24\%          & 66.78\%           & \textbf{54.67\%} & 40.37\%          & \textbf{33.79\%}            \\
\multicolumn{1}{c|}{Randomized Smoothing: $\sigma$ = 0.5}  & 96.28\%          & \textbf{83.28\%} & \textbf{68.17\%} & 53.86\%          & \textbf{48.79\%} & \multicolumn{1}{l}{33.10\%} \\
\multicolumn{1}{c|}{Randomized Smoothing: $\sigma$ = 1}    & 88.21\%          & 74.39\%          & 54.44\%          & 45.44\%          & 40.48\%          & 29.06\%                     \\ \bottomrule
\end{tabular}
\end{table}









\begin{table}[H]
\centering
\caption{30 PGD of Sticker Retraining against Adversarial Patch}
\label{tab:30sticker_sign_patch}
\begin{tabular}{ccccccc}
\toprule
                                                        & \multicolumn{6}{c}{Attacking Region}                                                                                       \\ \cmidrule(l){2-7} 
                                                        & 0\%              & 5\%              & 10\%             & 15\%             & 20\%             & 25\%                        \\ 
  \midrule
\multicolumn{1}{c|}{Clean Model}                        & \textbf{98.69\%} & 75.87\%          & 58.62\%          & 40.68\%          & 33.10\%          & 22.47\%                     \\
\multicolumn{1}{c|}{($10\times5$)Exhaustive Search}     & 95.38\%          & \textbf{91.46\%} & 86.67\%          & 76.39\%          & 68.12\%          & 55.57\%                     \\
\multicolumn{1}{c|}{($10\times5$)Gradient Based Search} & 95.30\%          & 86.67\%          & 80.57\%          & 75.00\%          & 64.90\%          & \multicolumn{1}{l}{54.44\%} \\
\multicolumn{1}{c|}{($7\times7$)Exhaustive Search}      & 93.99\%          & 89.02\%          & 82.93\%          & 78.40\%          & 66.90\%          & 55.92\%                     \\
\multicolumn{1}{c|}{($7\times7$)Gradient Based Search}  & 95.82\%          & 90.68\%          & \textbf{88.41\%} & \textbf{81.79\%} & \textbf{72.30\%} & \textbf{58.71\%}          \\ \bottomrule
\end{tabular}
\end{table}








\begin{table}[H]
\centering
\caption{50 PGD of Sticker Retraining against Adversarial Patch}
\label{tab:50sticker_sign_patc}
\begin{tabular}{@{}ccccccc@{}}
\toprule
                                                        & \multicolumn{6}{c}{Attacking Region}                                                                                       \\ \cmidrule(l){2-7} 
                                                        & 0\%              & 5\%              & 10\%             & 15\%             & 20\%             & 25\%                        \\ \midrule
\multicolumn{1}{c|}{Clean Model}                        & \textbf{98.69\%} & 75.87\%          & 58.62\%          & 40.68\%          & 33.10\%          & 22.47\%                     \\
\multicolumn{1}{c|}{($10\times5$)Exhaustive Search}     & 97.30\%          & \textbf{93.90\%} & 90.42\%          & 80.66\%          & 67.77\%          & 53.92\%                     \\
\multicolumn{1}{c|}{($10\times5$)Gradient Based Search} & 95.12\%          & 90.33\%          & 85.80\%          & 79.79\%          & 69.86\%          & \multicolumn{1}{l}{49.74\%} \\
\multicolumn{1}{c|}{($7\times7$)Exhaustive Search}      & 90.07\%          & 82.49\%          & 75.96\%          & 70.99\%          & 60.10\%          & 52.53\%                     \\
\multicolumn{1}{c|}{($7\times7$)Gradient Based Search}  & 95.82\%          & 90.33\%          & \textbf{89.29\%} & \textbf{78.92\%} & \textbf{70.21\%} & \textbf{58.54\%}            \\ \bottomrule
\end{tabular}
\end{table}

==> cadvadd.tex <==
\section{Additional Experiment on Curriculum Adversarial Training against Physically Realizable Attack}
\label{S:addcadv}

\begin{figure}[H]
\centering 
\label{100exs_glassAttAll}
\includegraphics[width=0.49\textwidth]{Figure/C50Adv_glassAttAll.pdf}
\caption{ Curriculum adversarial training with 50 iterations PGD against physically realizable attack}
\label{F:cadv50}
\end{figure}


==> evaluation.tex <==
\section{Evaluation}
In this section, we will evaluate the performance of current state-of-the-art robust model, adversarial training and randomized smoothing, against physical realizable attacks. We consider two tasks which are glass frame attacks on face recognition system as well as sticker attacks on the traffic sign. 

\subsection{Face recognition Setting}
We followed the exact same physical \citep{Sharif16} dodge attacks (untargeted attacks) on the face recognition systems (FRS).  They assume that the attacker who gains access to the FRS after the system has been trained, which is also classified as decision time attack and white-box scenario. To calculate the perturbations on the glass frame, they solved the optimization problem by gradient descent with momentum. It is an commonly used iterative algorithm that can minimize the objective function.

For the model, \citep{Parkhi2015DeepFR} has developed a 39-layer CNN (same as VGG-16 structure) for face recognition that achieved state-of-the-art performance on the Labeled Faces in the Wild (LFW)  challenge, a benchmark for testing Face Recognition Systems (FRS). The model was primarily set to recognize 2622 celebrities and achieved a classification accuracy around 98.95\%. In our case, instead of exploring such a huge dataset, we actually choose 10 subjects and do standard transfer learning. To be specific, those ten subjects are Buckley, Rahman, Khan, Staton, Tveit, Yoo, Cornish, Ferrara, Breslin and Spencer. All of the subjects have 300 to 500 images. In total, the data set has 3178 images on training set, 922 images on the validation set and 470 images on the test set. For our own transfer learning model, we customized fully connected layer of \citep{Parkhi2015DeepFR} model which reduced the output from 2422 to 10. We also used the pre-trained weights on convolution layers to train our model which achieved a classification accuracy of 99.36 \% on the test set after 30 epochs with ADAM optimizer. 

Besides, in our experiments, we use the same eyeglass frames with \citep{Sharif16} depicted in Fig.1. The frames occupy about 6.5\% of the pixels of the $224 \times 224$ face images, similarly to real frames. 

\begin{figure}[h]
\begin{center}
\includegraphics[width=0.3\linewidth]{Figure/glass.png}
\caption{The eyeglass frames used to fool FRSs (before
texture perturbation). By Clker-Free-Vector-Images / CC0
/ https://goo.gl/3RHKZA.}
\label{fig:Generate figure}
\end{center}
\end{figure}

\begin{figure}[H]
\begin{center}
\includegraphics[width=0.8\linewidth]{Figure/glass_example.png}
\caption{An example of the Glass Frame Attack. }
\label{fig:Generate figure}
\end{center}
\end{figure}

Figure 2 shows an example of glass frame attack. From left to right, they are Dave Annable, Dave Annable wearing adversarial glass frame and Allahrakka Rahman. The Model will predict the first picture as Dave Annable with 99 \% confidence and second picture as Allahrakka Rahman with 99.9\% confidence. The middle picture also gave you a sense how much our adversarial examples could take.\\

\subsection{Traffic Signs Setting}
Following the sticker attacks \citep{Eykholt2018RobustPA}, we also explored another dataset called LISA which contained 47 different U.S. traffic signs \citep{Mgelmose2012VisionBasedTS}. To alleviate the problem of imbalance and extremely blur data, we picked 16 best quality signs with 3509 training data and 1148 validation data in total after resizing to $32 \times 32$ pixels. Using LISA-CNN architecture defined in \citep{Eykholt2018RobustPA}, we successfully trained a classifier containing three convolutional layers and one FC layer with accuracy of 98.34 \% on the validation set. 

In this case, another optimization technique, ADAM optimizer \citep{Kingma2015AdamAM}, was implemented to solve the optimization problem. We also applied the the same sticker with \citep{Eykholt2018RobustPA}, which is a region resembling graffiti showed in Figure 3(b). 

\begin{figure}[H]
\centering 
\subfigure[Clean Stop Sign]{
\label{Fig.sub.1}
\includegraphics[width=0.25\textwidth]{Figure/clean_stopsign.png}}
\subfigure[Sticker Mask]{
\label{Fig.sub.2}
\includegraphics[width=0.25\textwidth]{Figure/stopsignmask.png}}
\subfigure[Stop Sign after Attacks]{
\label{Fig.sub.3}
\includegraphics[width=0.25\textwidth]{Figure/noise_stopsign.png}}
\caption{Example of Sticker Attack on Stop Sign}
\label{Fig.main}
\end{figure}

\subsection{Results for Face Dataset}
\subsubsection{Adversarial Training on Face Recognition}
We deploy the method of  \citep{madry2018towards} using $\epsilon = 4/255 $ \& $  8/255$ with both 7 and 50 iterations of PGD. In practice, it is quite hard to directly train a neural network using adversarial training in $224 \times 224$ case, especially when the allowed perturbations of adversaries are large. We tried to increase the $\epsilon$ to be $16/255$, but failed to make the model converge. 

We choose $\epsilon/4$ as $\alpha$ value for 7 iterations of PGD and 1/255 for 50 ones,  randomly start the initial perturbations and retrain the model for 30 epochs with ADAM optimizer. We use these models to test the performance against physically realizable attacks (Glass Frame Attacks). We follow the \citep{Sharif16} algorithm and pick the same learning rate 20/255 as well as momentum value 0.4. We also use the maximum iterations of 300 to test the models.

\begin{figure}[H]
\centering 
\label{Adv_glassAttAll}
\includegraphics[width=0.49\textwidth]{Figure/DiffIters_glassAll.pdf}
\label{Adv_glassAttFirst}
\includegraphics[width=0.49\textwidth]{Figure/DiffIters_glassFirst.pdf}
\caption{ Adversarial Training against Glass Frame Attacks on Face Recognition. The left plot shows results with 0 to 300 attack iterations. The right plot zooms in on the results with 0 to 20 attack iterations.}
\label{Adversarial Training against Glass Frame }
\end{figure}



We then borrow the ideas from curriculum adversarial training \citep{Cai18} which is training the model with weaker adversaries initially and then gradually improving the attack strength until it achieved limit. By this method, we develop the first model with $\epsilon = 4/255$ adversaries on top of clean model. After that, we retrain the previous model with $2 \ \times$ previous $\epsilon$. Hence, there are four different adversarial models in total with largest $\epsilon = 4/255, 8/255, 16/255$ and $32/255$. The adversaries were constructed in 7 iterations of PGD.



\begin{figure}[H]
\centering 
\label{Linf_glassAttAll}
\includegraphics[width=0.49\textwidth]{Figure/CAdv_glassAttAll.pdf}
\label{Linf_glassAttFirst}
\includegraphics[width=0.49\textwidth]{Figure/CAdv_glassAttFirst.pdf}
\caption{Curriculum Adversarial Training against Glass Frame Attacks on Face Recognition. The left plot shows results with 0 to 300 attack iterations. The right plot zooms in on the results with 0 to 20 attack iterations.}
\label{Curriculum Adversarial Training against Glass Frame }
\end{figure}

Figure \ref{Curriculum Adversarial Training against Glass Frame } shows the results of Adversarial Training against Glass Frame Attacks (GF). Adversarial Training models  have better robustness compared to original model. When the $\epsilon$ of adversaries increase, the performance of defending strong GF attacks improve. However, we notice that the model (which trained with higher $\epsilon$) tends to do worse in the lower iteration GF attacks. Generally, we are not satisfied with the adversarial training.

\begin{figure}[H]
\centering 
\label{CAcom_glassAttAll}
\includegraphics[width=0.49\textwidth]{Figure/CAcompare_glassAll.pdf}
\label{CAcom_glassAttFirst}
\includegraphics[width=0.49\textwidth]{Figure/CAcompare_glassFirst.pdf}
\caption{Comparison between two types of Training against Glass Frame Attacks on Face Recognition (omitting some bad cases). The left plot shows results with 0 to 300 attack iterations. The right plot zooms in on the results with 0 to 20 attack iterations.}
\label{Comparsion Adversarial Training against Glass Frame }
\end{figure}


\subsubsection{Randomized Smoothing on Face Recognition}

We choose the noise level $\sigma = 0.25, 0.5$, and $1$ (\ref{eqn:RS}) as \cite{Cohen2019CertifiedAR}. Then we use those three models to predict the test data under  Glass Frame attacks with 1,000 Monte Carlo samplings. We sample the images after attacks for 1000 times and use the base classifier to predict the images. Note that this method is provably robust against $l_2$ attacks.

\begin{figure}[H]
\centering 
\label{RS_glassAttAll}
\includegraphics[width=0.49\textwidth]{Figure/RS_glassAttAll.pdf}
\label{RS_glassAttFirst}
\includegraphics[width=0.49\textwidth]{Figure/RS_glassAttFirst.pdf}
\caption{Randomized Smoothing against Glass Frame Attacks on Face Recognition. The left plot shows results with 0 to 300 attack iterations. The right plot zooms in on the results with 0 to 20 attack iterations.}
\label{RS against Glass Frame }
\end{figure}

Generally, as Figure \ref{RS against Glass Frame } depicts, Randomized Smoothing has only limited improvement against the Glass Frame attacks even less effective than adversarial training. 

\subsection{Results for Traffic Sign Dataset}
\subsubsection{Adversarial Training on Traffic Sign}
Basically, we repeat the exactly same procedures with Face dataset in training adversarial models. Following \citep{Eykholt2018RobustPA}, we use 40 stop signs as our test data and do untargeted attacks.  we apply same settings with their attacks and use ADAM optimizer with same parameters. All the adversaries are constructed with 7 iterations PGD. 

\begin{table}[H]
\centering
\caption{ Adversarial Training against Sticker Attacks on Stop Sign
}
\label{tab:sign_A_sticker}
\begin{tabular}{@{}ccccc@{}}
\toprule
\multirow{2}{*}{\textbf{}}                              & \multicolumn{4}{c}{Attack Iterations}                              \\ \cmidrule(l){2-5} 
                                                        & $0$         & $10^1$          & $10^2$        & $10^3$          \\ \midrule
\multicolumn{1}{c|}{Clean Model}                        & \textbf{100\%} & 42.5\%          &  \textbf{32.5\% }       & 25\%            \\
\multicolumn{1}{c|}{Adv. Training: $\epsilon = 4/255$}  & \textbf{100\%}      & 42.5\%            & 25\%          & 27.5\%          \\
\multicolumn{1}{c|}{Adv. Training: $\epsilon = 8/255$}  & \textbf{100\% }        &  \textbf{50\%  }          & 30\%        & \textbf{ 32.5\%   }         \\
\multicolumn{1}{c|}{Adv. Training: $\epsilon = 16/255$} &  \textbf{100\% }        & 42.5\%     & 25\%     & 27.5\% \\
\multicolumn{1}{c|}{Adv. Training: $\epsilon = 32/255$} & 0\%          & 0\%           & 0\%         & 0\%           \\ \bottomrule
\end{tabular}
\end{table}


\begin{table}[H]
\centering
\caption{Curriculum Adversarial Training against Sticker Attacks on Stop Sign
}
\label{tab:sign_CA_sticker}
\begin{tabular}{@{}ccccc@{}}
\toprule
\multirow{2}{*}{\textbf{}}                              & \multicolumn{4}{c}{Attack Iterations}                              \\ \cmidrule(l){2-5} 
                                                        & $0$         & $10^1$          & $10^2$        & $10^3$          \\ \midrule
\multicolumn{1}{c|}{Clean Model}                        & \textbf{100\%} & 42.5\%          & 32.5\%        & 25\%            \\
\multicolumn{1}{c|}{CAdv. Training: $\epsilon = 4/255$}  & \textbf{100\%} & 35\%            & 25\%          & 22.5\%          \\
\multicolumn{1}{c|}{CAdv. Training: $\epsilon = 8/255$}  & 87.5\%         & 35\%            & 17.5\%        & 20\%            \\
\multicolumn{1}{c|}{CAdv. Training: $\epsilon = 16/255$} & 97.5\%         & \textbf{57.5\%} & \textbf{45\%} & \textbf{42.5\%} \\
\multicolumn{1}{c|}{CAdv. Training: $\epsilon = 32/255$} & 7.5\%          & 2.5\%           & 2.5\%         & 2.5\%           \\ \bottomrule
\end{tabular}
\end{table}

We notice that the best result of adversarial training as well as curriculum adversarial training, improve 10 \% to 20 \% of accuracy against the sticker attacks. However, it will be still attacked with high probability. Note that, for the adversaries with $\epsilon = 32/255$, we cannot make the model converge resulting very bad performance. 

\subsubsection{Randomized Smoothing on Traffic Sign}

In experiment, We find that Randomized Smoothing perform inconsistent against sticker attacks and largely depend on the base classifiers we train. Hence, to alleviate the problem, we use 5 random seed to repeat the experiment and use their mean values to denote the final results. 


\begin{table}[H]
\centering
\caption{Randomized Smoothing against Sticker Attacks on Stop Sign
}
\label{tab:sign_rs_sticker}
\begin{tabular}{@{}ccccc@{}}
\toprule
\multirow{2}{*}{\textbf{}}                                 & \multicolumn{4}{c}{Attack Iterations}                              \\ \cmidrule(l){2-5} 
                                                           & $0$         & $10^1$        & $10^2$          & $10^3$          \\ \midrule
\multicolumn{1}{c|}{Clean Model}                           & \textbf{100\%} & 42.5\%        & 32.5\%          & 25\%            \\
\multicolumn{1}{c|}{Randomized Smoothing: $\sigma = 0.25$} & \textbf{100\%} & \textbf{70\%} & \textbf{64.5\%} & \textbf{62.5\%} \\
\multicolumn{1}{c|}{Randomized Smoothing: $\sigma = 0.5$}  & 85.5\%         & 62.5\%        & 55\%            & 57.5\%          \\
\multicolumn{1}{c|}{Randomized Smoothing: $\sigma = 1$}    & 73\%           & 50.5\%        & 47.5\%          & 49.5\%          \\ \bottomrule
\end{tabular}
\end{table}

From Table \ref{tab:sign_rs_sticker}, Randomized Smoothing with $\sigma = 0.25$ improves the robustness a lot generally. However, it suffers some shortages. Firstly, our setting is considered as white attacks, while the attackers only attacks the base classifier not the smooth classifier. The attackers does not take advantage of the sampling procedure of randomized smoothing. Hence, the attacks are not what we considered the strongest attacks. Secondly, it takes longer time to predict one image compared to common convolutional  neural networks because of Monte Carlo sampling. Such time limitations will affect the drive-by testing (video testing) which is another important testing in physical world.



==> glass_frame_retrain.tex <==
\newpage
\section{Comparison between Glass Frame Retraining and Sticker Retraining }

\begin{figure}[H]
\centering 
\includegraphics[width=0.49\textwidth]{Figure/GlassFrameRetraining_glassAtt.pdf}
\caption{Glass Frame Retraining}
\label{sticker_example }
\end{figure}


==> sticker_retrain.tex <==
\section{Sticker Retraining}
Generally, we are not satisfied with current state-of-the-art robust models against physically realizable attacks. In this section, we present our method, sticker retraining, as an effective defending method against physically realizable attacks. It is quite similar to adversarial training, but constructing different kinds of adversaries. Our basic idea is finding a adversarial sticker on top of the image which can best simulate the physically realizable attack and then retraining with those adversaries. Hence, our algorithm is composed with two parts which are searching the best position to put the sticker and applying PGD to vary the color of the sticker.

We come up with two methods to locate the position of the stickers, which are exhaustive searching and gradient based searching. Exhaustive searching will guarantee to find a sticker that has strongest attacking strength, while gradient based searching will speed up the searching algorithm a lot suffering a little downgrade of performance.

The exhaustive searching follows these steps and the details are summarized in Algorithm \ref{Exhaustive Searching}
\begin{enumerate}

\item Given the pretrained model, the shape of the sticker as well as the data. 

\item For single data point, move the sticker to generate adversarial examples and check the cross entropy loss.

\item Report the position which the adversaries have largest cross entropy loss.

\end{enumerate}

%\ $1.$ Given the pretrained model, the shape of the sticker as well as the data.  \\
%\ $2.$ For single data point, move the sticker to generate adversarial examples and check the cross entropy loss.\\
%\ $3.$ Report the position which the adversaries have largest cross entropy loss.\\

\begin{algorithm}[!htbp]
\caption{Locating Sticker with Exhaustive Searching for one data point}
\label{Exhaustive Searching}
\hspace*{\algorithmicindent} \textbf{Input:} \\
Data: \ $X_i, y_i$; \ \ \ \
Test data shape: \ $N\times N$; \ \ \ \
Target Model: \ $Model$; \ \ \ \
Stride: \ $S$ ; \\
\hspace*{\algorithmicindent} \textbf{Output:} \\
Best Sticker Position: $(j', k')$\\
1.\textbf{function} ExhaustiveSearching($Model,X_i,y_i,N,S$) \\
2.\ \ \ \ \textbf{for} j \textbf{in} range($N/S$) \textbf{do}: \\
3.\ \ \ \ \ \ \ \ \textbf{for} k \textbf{in} range($N/S$) \textbf{do}:\\
4.\ \ \ \ \ \ \ \ \ \ \ \ Generate the adversarial $X_{i}^{adv}$ image by: \\
5.\ \ \ \ \ \ \ \ \ \ \ \ put the sticker on the image where top-left corner at $(j*S,k*S)$; \\
6.\ \ \ \ \ \ \ \ \ \ \ \ \textbf{if} CrossEntropyLoss($Model(X_{i}^{adv}), y_i$) is higher than previous loss: \\
7.\ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \textbf{Update} $(j',k') = (j,k)$ \\
8.\ \ \ \ \ \ \ \ \ \textbf{end for} \\
9.\ \ \ \ \ \textbf{end for} \\
10.\ \ \ \textbf{return} $(j',k')$
\end{algorithm}

The exhaustive searching is starting with a sticker from the top and left corner (0,0), and moving it top to bottom, left to right using for loop. Note that, $N$ is the length of single image (assuming square) and $S$ denotes the stride (pixels that sticker will skip when moving). $j$ and $k$ are integers from 0 to $N/S$,  where we want $(j*S,k*S)$ can denote the sticker's top-left corner when moving the sticker. At last, we will find the best position to put a sticker.

However, exhaustive searching needs to calculate the cross-entropy loss a lot of times. Each time of calculating requires forward propagation of the whole neural network, which is extremely time consuming. Inspiring by the gradient of neural network w.r.t. the input may stand for the sensitivity of the input, we then come up another searching method based the gradient value.

\begin{algorithm}[!htbp]
\caption{Locating Sticker with Gradient Based Searching for one data point}
\label{Gradient Based Searching}
\hspace*{\algorithmicindent} \textbf{Input:} \\
Data: \ $X_i, y_i$; \ \ \ \
Test data shape: \ $N\times N$; \ \ \ \
Target Model: \ $Model$; \ \ \ \
Stride: \ $S$ ; \\
Number of Potential Candidates: \ $C$; \\
\hspace*{\algorithmicindent} \textbf{Output:} \\
Best Sticker Position: $(j', k')$\\
\\
1.\textbf{function} GradientBasedSearching($Model,X_i,y_i,N,S,C$)\\
2.\ \ \ \ Calculate the gradient $Grad$ of CrossEntropyLoss($Model(X_{i}), y_i$) w.r.t. $X_i$ \\
3.\ \ \ \  $\displaystyle \sJ, \sK$ = HelperSearching($Grad,N,S,C$)\\
4.\ \ \ \ \textbf{for} $j,k$ \textbf{in} $\displaystyle \sJ, \sK$ \textbf{do}:\\
5.\ \ \ \ \ \ \ \ Generate the adversarial $X_{i}^{adv}$ image by: \\
6.\ \ \ \ \ \ \ \ put the sticker on the image where top-left corner at $(j*S,k*S)$; \\
7.\ \ \ \ \ \ \ \  \textbf{if} CrossEntropyLoss($Model(X_{i}^{adv}), y_i$) is higher than previous loss: \\
8.\ \ \ \ \ \ \ \ \ \ \ \ \ \textbf{Update} $(j',k') = (j,k)$ \\
9.\ \ \ \ \ \textbf{end for} \\
10.\ \ \ \textbf{return} $(j',k')$\\

1.\textbf{function} HelperSearching($Grad,N,S,C$) \\
2.\ \ \ \ \textbf{for} j \textbf{in} range($N/S$) \textbf{do}: \\
3.\ \ \ \ \ \ \ \ \textbf{for} k \textbf{in} range($N/S$) \textbf{do}:\\
4.\ \ \ \ \ \ \ \ \ \ \ \ Calculate the Sensitivity value $L = \sum (Grad_{sticker})^2$ where top-left corner at $(j*S,k*S)$; \\
6.\ \ \ \ \ \ \ \ \ \ \ \ \textbf{if} the Sensitivity value $L$ is in top $C$ of previous values: \\
7.\ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ Put $(j,k)$ in $\displaystyle \sJ, \sK$ and discard $(j_s , k_s)$ with lowest $L$ \\
8.\ \ \ \ \ \ \ \ \ \textbf{end for} \\
9.\ \ \ \ \ \textbf{end for} \\
10.\ \ \ \textbf{return} $\displaystyle \sJ, \sK$
\end{algorithm}

Instead of just using cross entropy loss, Algorithm \ref{Gradient Based Searching} also take advantage of the gradient $Grad$ to select $C$ potential candidates. $Grad$ has same shape with $X_i$ which is $N \times N$, and we assume the values of $Grad$ related to vulnerability of the input image. In function HelperSearching, we calculate sum of square of $Grad$ values inside the sticker region as $L$. For the whole image, we want to select $C$ candidate sticker's positions where their related $L$ are top $C$ and put those positions $(j,k)$ in the set $\displaystyle \sJ, \sK$. Then by loop through $\displaystyle \sJ, \sK$, we search the best position with cross entropy loss.

Therefore, we only need to find the gradient of the neural network and calculate cross entropy loss for only $C$ times, leading to a fast and flexible algorithm. By varying the value $C$, we can adjust between higher performance and faster speed. Note that if $C$ equals to the total searching times of Exhaustive Searching, then two methods are equivalent.

After finding out the position for the sticker, we will apply Projected Gradient Descent to attack the image by only changing the sticker region. This is equivalent to Equation \ref{eqn:physical} and various iterations can also control the attacking strength. With those properly selected adversaries, sticker retraining actually outperform all other methods.

\subsection{Sticker Retraining on Face Dataset}

We fix the shape of the sticker to be a $100 \times 50$ rectangle or a $70 \times 70$ square which are around 10 \% of whole image showed in Figure \ref{sticker_example }. We choose Stride $S = 5$ and 50 iterations of PGD under the sticker with learning rate $\alpha = 255/64$ as our best case. When searching the sticker, we always make the sticker to be $255/2$ on all RGB channel since it makes easier to do PGD attacks. We do not choose to randomly start the noise as we use $255/2$ to pick positions which is already a good point to start. Specially for gradient based searching, we pick 30 as the number of potential candidate positions. We also use ADAM optimizer with learning rate of 0.0001 to retrain the model with original model. After only 5 epochs, we early stop the training to avoid overfitting. 

\begin{figure}[H]
\centering 
\includegraphics[width=0.3\textwidth]{Figure/sticker_example.pdf}
\caption{An Example of Sticker Retraining. Sticker size: $100 \times 50$}
\label{sticker_example }
\end{figure}

\begin{figure}[H]
\centering 
\label{Main_glassAttAll}
\includegraphics[width=0.49\textwidth]{Figure/Main_glassAll.pdf}
\label{Main_glassAttFirst}
\includegraphics[width=0.49\textwidth]{Figure/Main_glassFirst.pdf}
\caption{The Best Case of Different Methods against Glass Frame Attacks on Face Recognition. The left plot shows results with 0 to 300 attack iterations. The right plot zooms in on the results with 0 to 20 attack iterations.}
\label{Main against Glass Frame }
\end{figure}

In Figure \ref{Main against Glass Frame }, we chooses the best case for all methods. It shows that Sticker Retraining has dominate performance compared to Adversarial Training as well as Randomized Smoothing in both clean accuracy and robustness. Besides, gradient based searching does not have a lot of downgrades and it is twice faster than exhaustive searching. 

We also test the various iterations of PGD on stickers for both searching methods of Sticker Retraining. The parameters we choose are 7 iterations with $\alpha = 255/8$, 20 iterations with $\alpha = 255/16$, 30 iterations with $\alpha = 255/32$ and 50 iterations with $\alpha = 255/64$. Figure \ref{100PGD against Glass Frame } shows as the iterations of PGD on stickers increases, the performance gets better. Also, gradient based searching has comparable results with exhaustive searching . 

\begin{figure}[H]
\centering 
\label{100exs_glassAttAll}
\includegraphics[width=0.49\textwidth]{Figure/EXS_glassAtt.pdf}
\label{100gbs_glassAttFirst}
\includegraphics[width=0.49\textwidth]{Figure/GBS_glassAtt.pdf}
\caption{Different Iterations of PGD of $100 \times 50$ Sticker Retrain against Glass Frame Attacks on Face Recognition. The left plot shows results of Exhaustive Searching. The right plot shows Gradient Based Searching.}
\label{100PGD against Glass Frame }
\end{figure}

%In addition, we try to simplify the whole procedure by training the model with only pretrained weights and sticker adversaries, meaning that we just do sticker training. We just select the gradient based searching in the experiment as a faster method. As Figure \ref{ST_glassAtt} shows, when we use large number of PGD, the performance is closed to the best case of Sticker Retraining. 

%\begin{figure}[H]
%\centering 
%\includegraphics[width=0.49\textwidth]{Figure/ST_glassAtt.pdf}
%\caption{Different Iterations of PGD of Sticker Training against Glass Frame Attacks on Face Recognition. }
%\label{ST_glassAtt}
%\end{figure}

\begin{figure}[H]
\centering 
\label{70exs_glassAttAll}
\includegraphics[width=0.49\textwidth]{Figure/EXS70_glassAtt.pdf}
\label{700gbs_glassAttFirst}
\includegraphics[width=0.49\textwidth]{Figure/GBS70_glassAtt.pdf}
\caption{Different Iterations of PGD of $70 \times 70$ Sticker Retrain against Glass Frame Attacks on Face Recognition. The left plot shows results of Exhaustive Searching. The right plot shows Gradient Based Searching.}
\label{700PGD against Glass Frame }
\end{figure}


\begin{figure}[H]
\centering 
\label{exs_glassAttAll}
\includegraphics[width=0.49\textwidth]{Figure/Comshapeexh_glassAtt.pdf}
\label{700gbs_glassAttFirst}
\includegraphics[width=0.49\textwidth]{Figure/Comshapegrad_glassAtt.pdf}
\caption{Different Iterations of PGD of $70 \times 70$ Sticker Retrain against Glass Frame Attacks on Face Recognition. The left plot shows results of Exhaustive Searching. The right plot shows Gradient Based Searching.}
\label{700PGD against Glass Frame }
\end{figure}







\subsection{Sticker Retraining on Traffic Sign Dataset}
For Traffic Sign Dataset, we repeat the same procedure with Face Dataset, but choose different parameters. In practice, we find that the clean model of traffic sign is more vulnerable since it only contains four layers. Hence, we choose a $10 \times 5 $ stickers which is around 5 \% of whole image. Specially, we use 10 potential candidates for Gradient Based Searching and Stride of 2 for both methods. The setting for PGD (iterations and $\alpha$) are exactly same with Face dataset. We also compare all  method with their best cases in Table \ref{tab:Main_sticker}.

\begin{table}[H]
\centering
\caption{The Best Case of Different Methods against Sticker Attacks on Stop Sign
}
\label{tab:Main_sticker}
\begin{tabular}{@{}ccccc@{}}
\toprule
\multirow{2}{*}{\textbf{}}                                 & \multicolumn{4}{c}{Attack Iterations}                                \\ \cmidrule(l){2-5} 
                                                           & $0$         & $10^1$          & $10^2$          & $10^3$          \\ \midrule
\multicolumn{1}{c|}{Clean Model}                           & \textbf{100\%} & 42.5\%          & 32.5\%          & 25\%            \\
\multicolumn{1}{c|}{Adv. Training: $\epsilon = 16/255$}    & 97.5\%         & 57.5\%          & 45\%            & 42.5\%          \\
\multicolumn{1}{c|}{Randomized Smoothing: $\sigma = 0.25$} & \textbf{100\%} & 70\%            & 64.5\%          & 62.5\%          \\
\multicolumn{1}{c|}{Exhaustive Search with 20 PGD }         & \textbf{100\%} & \textbf{86\%} & \textbf{85\%} & \textbf{85\%} \\
\multicolumn{1}{c|}{Gradient Based Search with 20 PGD}      & \textbf{100\%} & 82.5\%            & 82.5\%            & 81.5\%            \\ \bottomrule
\end{tabular}
\end{table}

Therefore, Exhaustive Search with 20 PGD outperform all other methods and improve the robustness a lot. We also varies the iterations of PGD for both methods to see the relationship with model robustness.

\begin{table}[H]
\centering
\caption{Exhaustive Searching with different PGD against Sticker Attacks on Stop Sign
}
\label{tab:Exhaustive Searching}
\begin{tabular}{@{}ccccc@{}}
\toprule
\multirow{2}{*}{\textbf{}}                                 & \multicolumn{4}{c}{Attack Iterations}                                \\ \cmidrule(l){2-5} 
                                                           & $0$         & $10^1$          & $10^2$          & $10^3$          \\ \midrule
\multicolumn{1}{c|}{Clean Model}                           & \textbf{100\%} & 42.5\%          & 32.5\%          & 25\%            \\
\multicolumn{1}{c|}{Exhaustive Search with 7 PGD }         & \textbf{100\%}  & 73\% & 70.5\% & 71\%  \\
\multicolumn{1}{c|}{Exhaustive Search with 20 PGD }         & \textbf{100\%} & 86\% & \textbf{85\%} & \textbf{85\%} \\
\multicolumn{1}{c|}{Exhaustive Search with 30 PGD }         & \textbf{100\%}  & \textbf{86.5\%} & 84\% & 82.5\%  \\
\multicolumn{1}{c|}{Exhaustive Search with 50 PGD }         & \textbf{100\%}  & 77\% & 76.5\% & 73.5\%   \\ \bottomrule
\end{tabular}
\end{table}



\begin{table}[H]
\centering
\caption{Gradient Based Searching with different PGD against Sticker Attacks on Stop Sign
}
\label{tab:Gradient Based Search}
\begin{tabular}{@{}ccccc@{}}
\toprule
\multirow{2}{*}{\textbf{}}                                 & \multicolumn{4}{c}{Attack Iterations}                                \\ \cmidrule(l){2-5} 
                                                           & $0$         & $10^1$          & $10^2$          & $10^3$          \\ \midrule
\multicolumn{1}{c|}{Clean Model}                           & \textbf{100\%} & 42.5\%          & 32.5\%          & 25\%            \\
\multicolumn{1}{c|}{Gradient Based Search with 7 PGD }         & \textbf{100\%} & \textbf{83.5\%} & 78\% & 78\% \\
\multicolumn{1}{c|}{Gradient Based Search with 20 PGD }         & \textbf{100\%}  & 82.5\% & 81.5\% & 80.5\%  \\
\multicolumn{1}{c|}{Gradient Based Search with 30 PGD }         & \textbf{100\%}  & \textbf{83.5\%} & 79.5\% & 81\%  \\
\multicolumn{1}{c|}{Gradient Based Search with 50 PGD }         & \textbf{100\%}&  82.5\% & \textbf{82.5\%} & \textbf{81.5\%}   \\ \bottomrule
\end{tabular}
\end{table}


However, we do not find a particular trend with iterations of PGD and robustness. The reason may varies, but the most important part is the clean model only contains four layers which are not a common used deep neural network. The structure may cause the model hard to learn stronger attacks. Besides, 40 stop sign test data may cause statistical inconsistent.

Interestingly, we do one more experiment on gradient based searching, where we use $7 \times 7$ stickers instead of $10 \times 5$. We report the result in Table \ref{tab:7*7Gradient Based Search}.


\begin{table}[H]
\centering
\caption{(\textbf{$7 \times 7$})Exhaustive Searching with different PGD against Sticker Attacks on Stop Sign
}
\label{tab:7*7Exh Search}
\begin{tabular}{@{}ccccc@{}}
\toprule
\multirow{2}{*}{\textbf{}}                                 & \multicolumn{4}{c}{Attack Iterations}                                \\ \cmidrule(l){2-5} 
                                                           & $0$         & $10^1$          & $10^2$          & $10^3$          \\ \midrule
\multicolumn{1}{c|}{Clean Model}                           & \textbf{100\%} & 42.5\%          & 32.5\%          & 25\%            \\
\multicolumn{1}{c|}{Exhaustive Search with 7 PGD }         &  \textbf{100\%} & 86.5\% & 85\%  & 85\%  \\
\multicolumn{1}{c|}{Exhaustive Search with 20 PGD }         & \textbf{100\%}  & 83\% & 80\% & 79\%  \\
\multicolumn{1}{c|}{Exhaustive Search with 30 PGD }         & \textbf{100\%}  & \textbf{92\%} & \textbf{92}\% & \textbf{90.5}\%  \\
\multicolumn{1}{c|}{Exhaustive Search with 50 PGD }         & \textbf{100\%}& 89.5\% & 89\% & 88.5\% \\ \bottomrule
\end{tabular}
\end{table}



\begin{table}[H]
\centering
\caption{(\textbf{$7 \times 7$})Gradient Based Searching with different PGD against Sticker Attacks on Stop Sign
}
\label{tab:7*7Gradient Based Search}
\begin{tabular}{@{}ccccc@{}}
\toprule
\multirow{2}{*}{\textbf{}}                                 & \multicolumn{4}{c}{Attack Iterations}                                \\ \cmidrule(l){2-5} 
                                                           & $0$         & $10^1$          & $10^2$          & $10^3$          \\ \midrule
\multicolumn{1}{c|}{Clean Model}                           & \textbf{100\%} & 42.5\%          & 32.5\%          & 25\%            \\
\multicolumn{1}{c|}{Gradient Based Search with 7 PGD }         &  \textbf{100\%} & 81.5\% & 80\%  & 79.5\%  \\
\multicolumn{1}{c|}{Gradient Based Search with 20 PGD }         & \textbf{100\%}  & 83.5\% & 82.5\% & 83\%  \\
\multicolumn{1}{c|}{Gradient Based Search with 30 PGD }         & \textbf{100\%}  & \textbf{85\%} & \textbf{85.5}\% & \textbf{84}\%  \\
\multicolumn{1}{c|}{Gradient Based Search with 50 PGD }         & \textbf{100\%}& 81\% & 81\% & 81.5\% \\ \bottomrule
\end{tabular}
\end{table}

Surprisingly, Gradient Based Searching with 30 PGD has the best result of all methods on Traffic Sign Dataset.


